Stationarity of asymptotically flat non-radiating electrovacuum spacetimes

It is proven that a solution to the Einstein-Maxwell equations whose gravitational and electromagnetic radiation fields vanish is in fact stationary in a neighbourhood of spatial infinity. That is, if the Weyl and Faraday tensors decay suitably fast, then there exists a time-like Killing vector field in the region outside the bifurcate horizon of a sphere of sufficiently large radius. In particular, truly dynamical time-periodic electrovacuum spacetimes do not exist. This is an extension of earlier work by Alexakis and Schlue and Bi\v{c}\'{a}k, Sholtz and Tod to include electromagnetism.

==> minkowski1.tex <==
\begin{tikzpicture}[scale=1]	%minkowski1

  % axes
  \draw[->] (-5,-2) -- (-5,1) node[above] {$t'$};

 	%boundaries and horizon
	\draw (-3,-3) -- (-3, 3);
	\draw (3,-3) -- (3,3);
	\draw (0,-3) ellipse (3 and 1) ;
	\draw (0,0) ellipse (3 and 1);
	\draw (0,3) ellipse (3 and 1);
	
	\draw 	(-3,3)  node[left] {$t'=\frac{\pi}{2}$}		
			(-3,0)  node[left] {$t'=0$}
			(-3,-3) node[left] {$t'=-\frac{\pi}{2}$} ;
			
	\draw[line width=1.5pt] (-1.5,2.15) .. controls(1,0.5) and (5.4,1) .. (1.5,0.85) node[pos=.25,above]{$J^+$};	%up front
	\draw[line width=1.5pt] (-1.5,-3.85) .. controls(0.5,-3) and (5.5,-0.5)  .. (1.5,0.85) node[pos=.4,below]{$J^-$};%down front
	\draw[line width=1.5pt] (-1.5,2.15) .. controls(-4.85,1.5) and (-2,1.5) .. (1.5,0.85);	%up back
	\draw[line width=1.5pt] (-1.5,-3.85) .. controls(-4.8,-1) and (-2,0)  .. (1.5,0.85);%down back

	%Labels
	\fill (-1.5,2.15) circle (2pt) node[above] {$i^+$};
	\fill (-1.5,-3.85) circle (2pt) node[below] {$i^-$};
	\fill (1.5,0.85) circle (2pt) node[below left] {$i^0$};

	
	%filling
	\draw [line width=1.5pt, dashed](-1.5, 2.15) -- (-1.5,-3.85) node[pos=0.8, right] {$r'=0$}  ;
	\draw [line width=1.5pt, dashed](1.5,-2.15) -- (1.5,3.85) node[pos=0.9, left]{$r'=\pi$};
	

%\begin{comment}
	\draw (-1.25,2) -- (-1.25,-3.75) ;			%verticals RIGHT top -- down
	\draw (-1,1.85) -- (-1,-3.65) ;					
	\draw (-.75,1.7) -- (-.75,-3.5);
	\draw (-.5,1.6) -- (-.5,-3.4);
	\draw (-.25,1.5) -- (-.25,-3.3);
	\draw (0,1.4) -- (0,-3.1);					%0th
	\draw (.25,1.35) -- (.25,-3);
	\draw (.5,1.3) -- (.5,-2.85);
	\draw (.75,1.25) -- (.75,-2.7);
	\draw (1,1.2) -- (1,-2.6);					%1st
	\draw (1.25,1.15) -- (1.25,-2.4);					
	\draw (1.4,1.10) -- (1.4,-2.3);
	\draw (1.6,1.05) -- (1.6,-2.2);
	\draw (1.8,1) -- (1.8,-2);
	\draw (2,.95) -- (2,-1.9);					%2nd
	\draw (2.2,.93) -- (2.2,-1.75);					
	\draw (2.4,.91) -- (2.4,-1.5);
	\draw (2.6,.89) -- (2.6,-1.3);
	\draw (2.8,.87) -- (2.8,-1.1);
	\draw (2.95,.87) -- (2.95,-.7);

	\draw (2.9,.87) -- (2.9,0);				%back	RIGHT
	\draw (2.7,.86) -- (2.7,.2);					
	\draw (2.5,.85) -- (2.5,.4);
	\draw (2.3,.84) -- (2.3,.5);
	\draw (2.1,.83) -- (2.1,.6);
	\draw (1.9,.83) -- (1.9,.7);


	\draw (-1.75,2.1) -- (-1.75,-3.6);					%verticals LEFT top -- down
	\draw (-2,2.05) -- (-2,-3.4);
	\draw (-2.25,2) -- (-2.25,-3.1);
	\draw (-2.5,1.9) -- (-2.5,-2.8);					
	\draw (-2.75,1.85) -- (-2.75,-2.4);					
	\draw (-2.9,1.8) -- (-2.9,-2.1);					
	
	\draw (-2.85,1.6) -- (-2.85,-1.1);					% LEFT back
	\draw (-2.6,1.5) -- (-2.6,-.8);
	\draw (-2.35,1.45) -- (-2.35,-.6);
	\draw (-2.1,1.4) -- (-2.1,-.4);					
	\draw (-1.85,1.4) -- (-1.85,-.25);					
	\draw (-1.6,1.35) -- (-1.6,-0.1);					
	\draw (-1.35,1.3) -- (-1.35,0);					

	\draw (-1.1,1.25) -- (-1.1,0.05);					
	\draw (-.85,1.2) -- (-.85,0.15);					
	\draw (-.6,1.15) -- (-.6,0.25);					
	\draw (-.35,1.15) -- (-.35,0.35);					
	\draw (-.1,1.1) -- (-.1,0.4);					

	\draw (.15,1.05) -- (.15,0.5);					
	\draw (.4,1.05) -- (.4,0.6);					
	\draw (.65,1) -- (.65,0.65);					
	\draw (.9,.95) -- (.9,0.7);					
	\draw (1.15,.9) -- (1.15,0.8);					

\end{tikzpicture} 

==> minkowski2.tex <==
\begin{tikzpicture}[scale=1]		%minkowski2

  % axes
%  \draw[->] (-1,-3) -- (-1,3) node[above] {$t'$};
	\draw (-3,0) node {};
	%Labels
	\fill (0,4) circle (2pt) node[above] {$i^+$};
	\fill (0,-4) circle (2pt) node[below] {$i^-$};
	\fill (4,0) circle (2pt) node[right] {$i^0$};

 	%boundaries and horizon
	\draw [line width = 1.5pt, dashed] (0,-4) -- (0,4) node[pos=.5,sloped,above] {$r'=0$};
	\draw [line width = 1.5pt] (0,4) -- (4,0) node[pos=.5, above right]{$J^+$};
	\draw [line width = 1.5pt] (0,-4) -- (4,0) node[pos=.5, below right]{$J^-$};

	\draw [dashed](0,4) ..controls (1,0).. (0,-4);
	\draw [dashed](0,4) ..controls (2,0).. (0,-4);
	\draw [dashed](0,4) ..controls (3,0).. (0,-4);
	\draw [dashed](0,4) ..controls (4,0).. (0,-4);


	\draw [dotted](4,0) -- (0,0);
	\draw [dotted](4,0) ..controls (1.5,.8).. (0,1);
	\draw [dotted](4,0) ..controls (1.5,1.8).. (0,2);
	\draw [dotted](4,0) ..controls (1.5,-.8).. (0,-1);
	\draw [dotted](4,0) ..controls (1.5,-1.8).. (0,-2);

\end{tikzpicture}

==> schwarzschild.tex <==
\begin{tikzpicture}[scale=1.]


  % axes
  \draw[dotted, ->] (-5,0) -- (5,0) node[right] {$x''$};
  \draw[dotted, ->] (0,-3) -- (0,3) node[above] {$t''$};
  \draw (2.2,0) node{$I$};
  \draw (-1.8,0) node{$I'$};
  \draw (0,1.1) node{$II_B$};
  \draw (0,-1) node{$II_W$};

 	%boundaries and horizon
	\draw[line width=1.5pt] (-2,-2) -- (2,2) node[pos=0.7, sloped, below]{$r=2m$};
	\draw[line width=1.5pt] (-2,2) -- (2,-2) node[pos=0.3, sloped, below]{$r=2m$};
	\draw (-4,0) -- (-2,-2) node[pos=0.5, below left]{$J^-$};
	\draw (-4,0) -- (-2,2) node[pos=0.5, above left]{$J^+$};
	\draw (4,0) -- (2,2) node[pos=0.5, above right]{$J^+$};
	\draw (4,0) -- (2,-2) node[pos=0.5, below right]{$J^-$};
	\draw[line width=2pt,dashed] (-2,2) -- (2,2) node[pos=0.5, above] {$r=0$};
	\draw[line width=2pt,dashed] (-2,-2) -- (2,-2) node[pos=0.5, below]{$r=0$};
	\fill (2,2) circle (2pt) node[above] {$i^+$};
	\fill (-2,2) circle (2pt) node[above] {$i^+$};
	\fill (-2,-2) circle (2pt) node[below] {$i^-$};
	\fill (2,-2) circle (2pt) node[below] {$i^-$};
	\fill (4,0) circle (2pt) node[above right] {$i^0$};
	\fill (-4,0) circle (2pt) node[above] {$i^0$};

	%t and x constant fillings
%	\draw[dotted, line width=1.5pt] (-4,0) .. controls(-1,-2) and (1,2) .. (4,0);
%	\draw[dotted, line width=1.5pt] (-4,0) .. controls(1,2) and (-1,-2) .. (4,0);
	\draw[dotted] (0,0) .. controls(2,1) .. (4,0);	
	\draw[dotted] (0,0) .. controls(2,-1) .. (4,0);	
	\draw[dotted] (0,0) .. controls(-2,1) .. (-4,0);
	\draw[dotted] (0,0) .. controls(-2,-1) .. (-4,0);

	\draw[dashed] (2,-2) -- (2,2);	
	\draw[dashed] (2,-2) .. controls(1,0) .. (2,2);	
	\draw[dashed] (2,-2) .. controls(3,0) .. (2,2);	

	\draw[dashed] (-2,-2) -- (-2,2);	
	\draw[dashed] (-2,-2) .. controls(-1,0) .. (-2,2);	
	\draw[dashed] (-2,-2) .. controls(-3,0) .. (-2,2);	

	\draw[dashed] (-2,2) .. controls(0,1) .. (2,2);	
	\draw[dashed] (-2,2) .. controls(0,0.5) .. (2,2);	
	\draw[dashed] (-2,-2) .. controls(0,-1) .. (2,-2);	
	\draw[dashed] (-2,-2) .. controls(0,-0.5) .. (2,-2);	

\end{tikzpicture}
